Aligning Autoresearch: Co-Improvement between Agents and Humans

Autoresearch agents can now attempt long-horizon AI research end-to-end, i.e., self-improvement. However, best results are still obtained by research agents interacting with human researchers, and improving AI's ability to perform this co-research will only reinforce this effect---a process termed co-improvement (Weston and Foerster, 2025). Further, aligning with human expectations is likely a safer path for research agents, especially given recent agent reward hacking phenomena (OpenAI, 2026b). In this work we address these issues in four ways: (i) we empirically study the role of humans in directing autoresearch agents, focusing on the domain of benchmark creation, and find humans still play a pivotal role particularly in the ideation phase; (ii) we also develop a benchmark, HackBench, that shows current autoresearch agents are not aligned and are unable to achieve hack localization sufficiently; (iii) we present a method to train agents for improved human interaction by using human simulators as a proxy during reinforcement learning (RL); and finally (iv) we develop a method to improve model text generation, and hence agent communication, by RL with rubrics aligned with human experts. Together, our training and evaluation recipes provide a path toward more capable and aligned (co-)research agents.

==> scratch.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{2}{c}{Alpaca Eval 2.0} & \multicolumn{2}{c}{Arena Hard v2.0} & \multicolumn{1}{c}{NoveltyBench} \\ \cmidrule{2-6}
 & LCWR(\%) & WR(\%) & creative writing & hard prompts & Distinct (\#) \\
\midrule
Quality only       & 48.74 & 57.01 & 61.1 {\footnotesize(-3.5 / +4.5)} & 33.9 {\footnotesize(-2.3 / +2.5)} & 2.08 \\
Quality only (no norm)             & 52.57 & 61.18 & 68.1 {\footnotesize(-3.5 / +2.7)} & 24.7 {\footnotesize(-2.0 / +2.1)} & 2.28 \\
Quality + 4gram (additive)                             & 49.16 & 56.83 & 64.7 {\footnotesize(-3.2 / +2.6)} & 32.8 {\footnotesize(-2.6 / +2.2)} & 3.33 \\
Quality + 4gram (multiplicative)                       & 48.48 & 57.76 & 65.3 {\footnotesize(-3.3 / +3.6)} & \textbf{34.3} {\footnotesize(-1.7 / +3.2)} & 2.79 \\ \midrule
Quality + 4gram (multiplicative, no norm)              & \textbf{53.82} & \textbf{66.46} & \textbf{71.9} {\footnotesize(-3.3 / +3.6)} & 31.3 {\footnotesize(-2.3 / +2.9)} & \textbf{3.59} \\
\bottomrule
\end{tabular}
\caption{Evaluation results on Alpaca Eval 2.0, Arena Hard v2.0 (Official w/ Style Control), and NoveltyBench. The same checkpoint (1000 steps) is chosen for a fair comparison.}
\end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{2}{c}{Alpaca Eval 2.0} & \multicolumn{2}{c}{Arena Hard v2.0} & \multicolumn{1}{c}{NoveltyBench} \\ \cmidrule{2-6}
 & LCWR(\%) & WR(\%) & creative writing & hard prompts & Distinct (\#) \\
\midrule
\texttt{Llama-3.1-8B-Instruct} & 31.92 & 32.61 & 7.1 {\footnotesize{(-1.4 / +1.8)}} & 6.4 {\footnotesize{(-0.8 / +1.3)}} & 5.28 \\ 
\midrule
Quality only       & 48.74 & 57.01 & 61.1 {\footnotesize(-3.5 / +4.5)} & 33.9 {\footnotesize(-2.3 / +2.5)} & 2.08 \\
Quality only (no norm)             & 52.57 & 61.18 & 68.1 {\footnotesize(-3.5 / +2.7)} & 24.7 {\footnotesize(-2.0 / +2.1)} & 2.28 \\
Quality + 4gram (additive)                             & 49.16 & 56.83 & 64.7 {\footnotesize(-3.2 / +2.6)} & 32.8 {\footnotesize(-2.6 / +2.2)} & 3.33 \\
Quality + 4gram (multiplicative)                       & 48.48 & 57.76 & 65.3 {\footnotesize(-3.3 / +3.6)} & \textbf{34.3} {\footnotesize(-1.7 / +3.2)} & 2.79 \\ 
Quality + 4gram (multiplicative, no norm)              & \textbf{53.82} & \textbf{66.46} & \textbf{71.9} {\footnotesize(-3.3 / +3.6)} & 31.3 {\footnotesize(-2.3 / +2.9)} & \textbf{3.59} \\ 
\midrule
Quality + partition (additive)                         & 53.17 & 60.82 & 69.2 {\footnotesize(-3.6 / +3.9)} & 32.7 {\footnotesize(-3.2 / +2.9)} & 5.23 \\
Quality + partition (multiplicative)                   & 51.64 & 62.17 & \textbf{69.7} {\footnotesize(-3.3 / +4.0)} & \textbf{35.2} {\footnotesize(-2.6 / +2.5)} & 3.34 \\
Quality + partition (multiplicative, no norm)          & \textbf{55.15} & \textbf{65.34} & 68.8 {\footnotesize(-3.3 / +2.9)} & 31.1 {\footnotesize(-2.0 / +2.1)} & \textbf{5.49} \\
\bottomrule
\end{tabular}
\caption{Evaluation results on Alpaca Eval 2.0, Arena Hard v2.0 (with Style Control), and NoveltyBench. Judges are GPT-4o without chain of thought. \textbf{The checkpoint with the highest validation diversity is selected.}}
\end{table}


\begin{table}[htbp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l*{12}{c}}
        \toprule
        & \multicolumn{3}{c}{AIME24} & \multicolumn{3}{c}{AIME25} & \multicolumn{3}{c}{OlympiadBench} & \multicolumn{3}{c}{Avg.} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
        \texttt{pass@k} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} \\
        \midrule
        \textbf{Qwen3-4B-Base} 
        & 9.66 & 42.26 & 49.49 & 7.94 & 45.36 & 53.33 & 31.02 & 66.93 & 70.22 & 16.21 & 51.52 & 57.68 \\ \midrule
        GRPO
        & \textbf{21.20} & 51.27 & 56.64 & \textbf{17.08} & \textbf{54.15} & 60.01 & \textbf{43.70} & 68.70 & 71.11 & \textbf{27.33} & 58.04 & 62.59 \\
        GRPO-Unlikeliness    &  --- & --- & ---  & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
        %\textbf{4gram}
        %& \underline{18.41} & \underline{53.80} & \underline{63.14} & \underline{17.01} & 52.44 & \underline{61.52} & \underline{41.69} & \underline{69.20} & \underline{72.00} & \underline{25.70} & \underline{58.48} & \underline{65.55} \\
        %& \underline{18.41} & \underline{53.80} & \underline{63.14} & \underline{17.01} & 52.44 & \underline{61.52} & \underline{41.69} & \underline{69.20} & \underline{72.00} & \underline{25.70} & \underline{58.48} & \underline{65.55} \\
        \cellcolor{blue!10}\textbf{\method} (Ours)
        & \cellcolor{blue!10}16.95 & \cellcolor{blue!10}\textbf{57.60} & \cellcolor{blue!10}\textbf{66.71}
        & \cellcolor{blue!10}16.20 & \cellcolor{blue!10}\underline{53.96} & \cellcolor{blue!10}\textbf{63.30}
        & \cellcolor{blue!10}41.43 & \cellcolor{blue!10}\textbf{70.39} & \cellcolor{blue!10}\textbf{75.45}
        & \cellcolor{blue!10}24.86 & \cellcolor{blue!10}\textbf{60.65} & \cellcolor{blue!10}\textbf{68.49} \\ \midrule \midrule
                \textbf{Qwen3-14B-Base} 
        & 13.44 & 60.13 & 66.67 & 11.80 & 45.79 & 54.47 & 38.1 & 69.96 & 73.19 & --- & --- & --- \\ \midrule
        GRPO
        & \textbf{21.20} & 51.27 & 56.64 & \textbf{17.08} & \textbf{54.15} & 60.01 & \textbf{43.70} & 68.70 & 71.11 & \textbf{27.33} & 58.04 & 62.59 \\
        GRPO-Unlikeliness    &  --- & --- & ---  & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
        %\textbf{4gram}
        %& \underline{18.41} & \underline{53.80} & \underline{63.14} & \underline{17.01} & 52.44 & \underline{61.52} & \underline{41.69} & \underline{69.20} & \underline{72.00} & \underline{25.70} & \underline{58.48} & \underline{65.55} \\
        %& \underline{18.41} & \underline{53.80} & \underline{63.14} & \underline{17.01} & 52.44 & \underline{61.52} & \underline{41.69} & \underline{69.20} & \underline{72.00} & \underline{25.70} & \underline{58.48} & \underline{65.55} \\
        \cellcolor{blue!10}\textbf{\method} (Ours)
        & \cellcolor{blue!10}16.95 & \cellcolor{blue!10}\textbf{57.60} & \cellcolor{blue!10}\textbf{66.71}
        & \cellcolor{blue!10}16.20 & \cellcolor{blue!10}\underline{53.96} & \cellcolor{blue!10}\textbf{63.30}
        & \cellcolor{blue!10}41.43 & \cellcolor{blue!10}\textbf{70.39} & \cellcolor{blue!10}\textbf{75.45}
        & \cellcolor{blue!10}24.86 & \cellcolor{blue!10}\textbf{60.65} & \cellcolor{blue!10}\textbf{68.49} \\
        \bottomrule
    \end{tabular}
    \caption{Pass@k (\%) on three competition math benchmarks using \textbf{Qwen3-4B-Base} and \textbf{Qwen3-14B-Base} as the reference policy. Training dataset = DeepscaleR \citep{deepscaler2025}. Columns are grouped by benchmark with an additional Avg. (mean over AIME24, AIME25, OlympiadBench). \texttt{pass@\{1, 64, 128\}} is calculated over 256 generations (avg@256). The best score in each column is \textbf{bolded}. \textbf{\method~is able to greatly improve (+5.9\%) on \textbf{pass@\{64, 128\}} by increasing response diversity while slightly decreasing \textbf{pass@1}.}}
    \label{tab:math_pass_k_grouped_transposed}
\end{table}


\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{2}{c}{Alpaca Eval 2.0*} & \multicolumn{1}{c}{Arena Hard v2.0*} & \multicolumn{2}{c}{NoveltyBench} \\ \cmidrule(lr){2-3}  \cmidrule(lr){4-4} \cmidrule(lr){5-6}
 & LCWR(\%) & WR(\%) & Creative Writing (\%) & Distinct (\#) & Dist-4grams (\%) \\
\midrule
\textbf{Llama-3.1-8B-Instruct} & 31.92 & 32.61 & 7.1 {\footnotesize{(-1.4 / +1.8)}} & \underline{5.28} & 93.94 \\ \midrule
GRPO  & 48.74 & 57.01 & 61.1 {\footnotesize(-3.5 / +4.5)} & 2.08 & 92.84 \\
%GRPO\footnotesize{(w/o norm)}      & 52.57 & 61.18 & 68.1 {\footnotesize(-3.5 / +2.7)} & 2.28 & 94.05 \\
DivPO           & 43.53  & 43.17 &  --- & 4.34 & 94.12 \\
GRPO-Unlikeliness &  --- & --- & ---  & --- & --- \\
%GRPO $\times$ 4gram diversity              & 53.82 & \textbf{66.46} & \textbf{71.9} {\footnotesize(-3.3 / +3.6)} & 3.59 & \underline{95.63} \\ 
\rowcolor{blue!10}\method~(Ours)      & \textbf{55.15} & \textbf{65.34} & \textbf{68.8} {\footnotesize(-3.3 / +2.9)} & \textbf{5.49} & \textbf{96.04} \\ \midrule \midrule
\textbf{Llama-3.3-70B-Instruct} & 44.55 & 45.28 &  17.7 {\footnotesize(-2.9 / +2.7)} & 2.95 & 91.73 \\ \midrule
GRPO      & 73.27 & 90.00 & 89.7  {\footnotesize(-2.5 / +2.0)} & 2.31 & 94.58 \\
%GRPO\footnotesize{(w/o norm)}  & --- & --- & --- & --- & --- \\
DivPO &  --- & --- & ---  & --- & --- \\
GRPO-Unlikeliness    &  --- & --- & ---  & --- & --- \\
%GRPO $\times$ 4gram diversity & --- & --- & --- & --- & --- \\
\rowcolor{blue!10} \method~(Ours)     & \textbf{80.37} & \textbf{91.37} & \textbf{91.2} \footnotesize{(-2.0 / +1.5)} & \textbf{4.26} & \textbf{95.25} \\
\bottomrule
\end{tabular}
\caption{Non-verifiable Evaluations. For each method, we train a single model on 10,000 WildChat prompts. We evaluate the models on Alpaca Eval 2.0, Arena Hard v2.0 (creative writing subset with markdown and length style control), and NoveltyBench. * indicates we used GPT-4o as the judge. \textbf{Models trained with \method~achieve the best quality in terms of win rates in Alpaca Eval and Arena Hard, and simultaneously are the most diverse model on NoveltyBench.}}
\label{table:wildchat}
\end{table}


\begin{table}[htbp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l*{12}{c}}
        \toprule
        & \multicolumn{3}{c}{AIME24} & \multicolumn{3}{c}{AIME25} & \multicolumn{3}{c}{OlympiadBench} & \multicolumn{3}{c}{Avg.} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
        \texttt{pass@k} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} & \texttt{k=1} & \texttt{k=64} & \texttt{k=128} \\
        \midrule
        \textbf{Qwen3-4B-Base} 
        & 9.66 & 42.26 & 49.49 & 7.94 & 45.36 & 53.33 & 31.02 & 66.93 & 70.22 & 16.21 & 51.52 & 57.68 \\ \midrule
        GRPO
        & \textbf{23.20} & 57.51 & 62.17 & 20.57 & 53.47 & 55.62 & 45.24 & 69.41 & 71.41 & 29.67 & 60.13 & 63.07 \\
        GRPO-Unlikeliness    &  --- & --- & ---  & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
        %\textbf{4gram}
        %& \underline{18.41} & \underline{53.80} & \underline{63.14} & \underline{17.01} & 52.44 & \underline{61.52} & \underline{41.69} & \underline{69.20} & \underline{72.00} & \underline{25.70} & \underline{58.48} & \underline{65.55} \\
        %& \underline{18.41} & \underline{53.80} & \underline{63.14} & \underline{17.01} & 52.44 & \underline{61.52} & \underline{41.69} & \underline{69.20} & \underline{72.00} & \underline{25.70} & \underline{58.48} & \underline{65.55} \\
        \cellcolor{blue!10}\textbf{\method} (Ours)
        & \cellcolor{blue!10}20.57 & \cellcolor{blue!10}\textbf{58.66} & \cellcolor{blue!10}\textbf{64.15}
        & \cellcolor{blue!10}\textbf{21.30} & \cellcolor{blue!10}\textbf{55.23} & \cellcolor{blue!10}\textbf{56.77}
        & \cellcolor{blue!10}\textbf{47.11} & \cellcolor{blue!10}\textbf{71.30} & \cellcolor{blue!10}\textbf{73.78}
        & \cellcolor{blue!10}29.67 & \cellcolor{blue!10}\textbf{61.73} & \cellcolor{blue!10}\textbf{64.90} \\ \bottomrule
    \end{tabular}
    \caption{Pass@k (\%) on three competition math benchmarks using \textbf{Qwen3-4B-Base} and \textbf{Qwen3-14B-Base} as the reference policy. Training dataset = DAPO \citep{yu2025dapoopensourcellmreinforcement}. Columns are grouped by benchmark with an additional Avg. (mean over AIME24, AIME25, OlympiadBench). \texttt{pass@\{1, 64, 128\}} is calculated over 256 generations (avg@256). The best score in each column is \textbf{bolded}. \textbf{\method~is able to improve on \textbf{pass@\{64, 128\}} by increasing response diversity while slightly decreasing \textbf{pass@1}.}}
    \label{tab:math_pass_k_grouped_transposed_dapo}
\end{table}


==> unslop/metarubric_traj_table.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{ccccc}
    \toprule
    Iteration & train (blind) & val (blind) & train (GT) & val (GT) \\
    \midrule
    0 & $-2.02$ & $-2.81$ & $+0.02$ & $-0.69$ \\
    1 & $-1.51$ & $-2.12$ & $+0.83$ & $+0.65$ \\
    2 & $+0.10$ & $-0.31$ & $+1.55$ & $+1.73$ \\
    3 & $+0.80$ & $\mathbf{+0.41}$ & $+1.44$ & $+1.63$ \\
    \bottomrule
    \end{tabular}
    \caption{Meta-rubric optimization: mean gap (human $-$ Muse final score, 0--10
    scale) by iteration, split (train/val) and rubric variant (blind / GT-informed).
    The optimizer sees only the train split. The honest signal is \emph{val (blind)},
    which rises monotonically $-2.81\!\to\!+0.41$ and tracks the train column
    throughout (final spread $\approx 0.4$)---the learned meta-prompt generalizes to
    held-out papers rather than fitting the diagnosed ones.}
    \label{unslop:table:metarubric_traj}
\end{table}
